Visual cognition in multimodal large language models

A chief goal of artificial intelligence is to build machines that think like people. Yet it has been argued that deep neural network architectures fail to accomplish this. Researchers have asserted these models' limitations in the domains of causal reasoning, intuitive physics, and intuitive psychology. Yet recent advancements, namely the rise of large language models, particularly those designed for visual processing, have rekindled interest in the potential to emulate human-like cognitive abilities. This paper evaluates the current state of vision-based large language models in the domains of intuitive physics, causal reasoning, and intuitive psychology. Through a series of controlled experiments, we investigate the extent to which these modern models grasp complex physical interactions, causal relationships, and intuitive understanding of others' preferences. Our findings reveal that, while some of these models demonstrate a notable proficiency in processing and interpreting visual data, they still fall short of human capabilities in these areas. Our results emphasize the need for integrating more robust mechanisms for understanding causality, physical dynamics, and social cognition into modern-day, vision-based language models, and point out the importance of cognitively-inspired benchmarks.

==> dump.tex <==
%Numerous studies have investigated the reasoning capabilities of modern large language models. While most previous studies are in the text domain only, the advent of new multimodal LLMs opens up new opportunities for assessing their capabilities. Inspired by previous works that employ methods and stimuli from cognitive science and psychology to better understand LLMs \cite{binz2022using, akata2023playing}, we here use visual stimuli from cognitive science experiments to investgiate three core components required for building human-like artificial intelligence as outlined by \cite{lake2017building}: intuitive physics, causality, and intuitive psychology. 

%\citep{baillargeon1996infants} outlines different experiments that can be used to investigate intuitive physical understanding. Chief among these is "support events", where different objects are stacked on top of each other in stable or unstable configurations. These types of stimuli have also been used in machine learning research in order to test the intuitive physical understanding of neural networks (see \citep{buschoff2023acquisition} for an overview on previous work on building models with human-like physical knowledge). Most previous approaches rely on a simulation based physics engine \citep{battaglia2013simulation, battaglia2016interaction, smith2019modeling}. In contrast, \citep{lerer2016learning} use large convolutional networks to predict binary stability judgements of block towers as well as the trajectories of falling blocks. They showed that the performance of such networks exceeds that of human subjects on synthetic data. 
